Parameterizing empirical interatomic potentials for predicting thermophysical properties via an irreducible derivative approach: the case of ThO$_2$ and UO$_2$

The accuracy of classical physical property predictions using molecular dynamics simulations is determined by the quality of the interatomic potentials. Here we introduce a training approach for empirical interatomic potentials (EIPs) which is well suited for capturing phonons and phonon-related properties. Our approach is based on direct comparisons of the second- and third-order irreducible derivatives between an EIP and the Born-Oppenheimer potential within density functional theory (DFT) calculations. Irreducible derivatives fully exploit space group symmetry and allow for training without redundant information. We demonstrate the fidelity of our approach in the context of ThO$_2$ and UO$_2$, where we optimize parameters of an embedded-atom method potential in addition to core-shell interactions. Our EIPs provide thermophysical properties in good agreement with DFT and outperform widely utilized EIPs for phonon dispersion and thermal conductivity predictions. Reasonable estimates of thermal expansion and formation energies of Frenkel pairs are also obtained.

==> tables/table_lattice_constant.tex <==
\begin{ruledtabular}
\begin{tabular}{@{}cccc}
\textrm{}& $a(0K) (\AA)$ & $a(300K) (\AA)$ & $q_{Th}^{eff}(|e|)$  \\
\hline\hline \\[-0.8em]
\multicolumn{4}{c}{ThO$_2$}\\[0.2em]
\colrule\\[-0.8em]
SCAN & 5.592 & -     & 2.447  \\[0.2em]
CRG  & 5.580 & 5.595 & 2.221  \\[0.2em]
PW   & 5.592 & 5.607 & 2.447  \\[0.2em]
EXP  &   -   & 5.600 \cite{idiri_behavior_2004}, 5.597 \cite{hirata_high_1977} & xxx  \\[0.8em]

\multicolumn{4}{c}{UO$_2$}\\[0.2em]
\colrule\\[-0.8em]
PBE  & 5.546 & -     & 2.325  \\[0.2em]
CRG  & 5.453 & 5.467xxx & 2.221  \\[0.2em]
PW   & 5.546 & xxx & 2.325  \\[0.2em]
EXP  &   -   & xxx & xxx  
\end{tabular}
\end{ruledtabular}

==> tables/table_sm_ids_of_2si.tex <==
\begin{ruledtabular}
\begin{tabular}{@{}lcl}
\\[-1.0em]
$\CMcal{Q}$  & Count & Derivatives \\ [0.2em]
\hline\hline \\[-0.8em]
\multicolumn{3}{c}{Irreducible derivatives for $\CMcal{N}=2$, $ \mathbf{\hat{S}}_\mathrm{BZ}=2\mathbf{\hat{S}}_\mathrm{I}$ }\\[0.2em]
\colrule  \\[-0.8em]
$(\Gamma,\Gamma)$ & 2 & 
$d\indices*{*_{\Gamma}^{T_{2g}^{}}_{\Gamma}^{T_{2g}^{}}}$,
$d\indices*{*_{\Gamma}^{T_{1u}^{}}_{\Gamma}^{T_{1u}^{}}}$ \\ [0.4em]
$(X,X)$ & 7 & 
$d\indices*{*_{X}^{A_{1g}^{}}_{X}^{A_{1g}^{}}}$,
$d\indices*{*_{X}^{E_{g}^{}}_{X}^{E_{g}^{}}}$,
$d\indices*{*_{X}^{A_{2u}^{}}_{X}^{A_{2u}^{}}}$,
$d\indices*{*_{X}^{B_{1u}^{}}_{X}^{B_{1u}^{}}}$,
$d\indices*{*_{X}^{E_{u}^{}}_{X}^{E_{u}^{}}}$,
$d\indices*{*_{X}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}_{X}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}}$,
$d\indices*{*_{X}^{E_{u}^{}}_{X}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}}$\\[0.8em]
\iffalse
$(L,L)$ & 8 & 
$d\indices*{*_{L}^{A_{1g}^{}}_{L}^{A_{1g}^{}}}$,
$d\indices*{*_{L}^{\tensor*[^{1}]{\hspace{-0.2em}A}{}_{1g}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}A}{}_{1g}^{}}}$,
$d\indices*{*_{L}^{A_{1g}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}A}{}_{1g}^{}}}$,
$d\indices*{*_{L}^{E_{g}^{}}_{L}^{E_{g}^{}}}$,
$d\indices*{*_{L}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}}$,
$d\indices*{*_{L}^{E_{g}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}}$,
$d\indices*{*_{L}^{A_{2u}^{}}_{L}^{A_{2u}^{}}}$,
$d\indices*{*_{L}^{E_{u}^{}}_{L}^{E_{u}^{}}}$ \\[0.8em]
\fi
\multicolumn{3}{c}{Irreducible derivatives for $\CMcal{N}=3$, $ \mathbf{\hat{S}}_\mathrm{BZ}=2\mathbf{\hat{S}}_\mathrm{I}$ }\\[0.2em]
\colrule\\[-0.8em]
$(\Gamma,\Gamma,\Gamma)$ & 2 &  
$d\indices*{*_{\Gamma}^{T_{2g}^{}}_{\Gamma}^{T_{2g}^{}}_{\Gamma}^{T_{2g}^{}}}$,
$d\indices*{*_{\Gamma}^{T_{1u}^{}}_{\Gamma}^{T_{1u}^{}}_{\Gamma}^{T_{2g}^{}}}$ \\
\\[-0.8em]
\iffalse
$(\Gamma,L,L)$ & 27 & \makecell{ 
$d\indices*{*_{\Gamma}^{T_{2g}^{}}_{L}^{A_{1g}^{}}_{L}^{A_{1g}^{}}}$,                       
$d\indices*{*_{\Gamma}^{T_{2g}^{}}_{L}^{A_{1g}^{}}_{L}^{E_{g}^{}}}$,                                                  
$d\indices*{*_{\Gamma}^{T_{2g}^{}}_{L}^{A_{1g}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}A}{}_{1g}^{}}}$,
$d\indices*{*_{\Gamma}^{T_{2g}^{}}_{L}^{A_{1g}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}}$,
$\tensor*[^{0}]{d}{}\indices*{*_{\Gamma}^{T_{2g}^{}}_{L}^{E_{g}^{}}_{L}^{E_{g}^{}}}$,                                 
$\tensor*[^{0}]{d}{}\indices*{*_{\Gamma}^{T_{2g}^{}}_{L}^{E_{g}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}}$,
$\tensor*[^{1}]{d}{}\indices*{*_{\Gamma}^{T_{2g}^{}}_{L}^{E_{g}^{}}_{L}^{E_{g}^{}}}$,                                   
$d\indices*{*_{\Gamma}^{T_{2g}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}A}{}_{1g}^{}}_{L}^{E_{g}^{}}}$,\\
$\tensor*[^{1}]{d}{}\indices*{*_{\Gamma}^{T_{2g}^{}}_{L}^{E_{g}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}}$,                
$d\indices*{*_{\Gamma}^{T_{2g}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}A}{}_{1g}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}A}{}_{1g}^{}}}$,                 
$d\indices*{*_{\Gamma}^{T_{2g}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}A}{}_{1g}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}}$,
$\tensor*[^{0}]{d}{}\indices*{*_{\Gamma}^{T_{2g}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}}$, 
$\tensor*[^{1}]{d}{}\indices*{*_{\Gamma}^{T_{2g}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}}$,
$d\indices*{*_{\Gamma}^{T_{2g}^{}}_{L}^{A_{2u}^{}}_{L}^{A_{2u}^{}}}$,                                                               
$d\indices*{*_{\Gamma}^{T_{2g}^{}}_{L}^{A_{2u}^{}}_{L}^{E_{u}^{}}}$,                                                                  
$\tensor*[^{0}]{d}{}\indices*{*_{\Gamma}^{T_{2g}^{}}_{L}^{E_{u}^{}}_{L}^{E_{u}^{}}}$, \\                                              
$\tensor*[^{1}]{d}{}\indices*{*_{\Gamma}^{T_{2g}^{}}_{L}^{E_{u}^{}}_{L}^{E_{u}^{}}}$,                                
$d\indices*{*_{\Gamma}^{T_{1u}^{}}_{L}^{A_{1g}^{}}_{L}^{A_{2u}^{}}}$,
$d\indices*{*_{\Gamma}^{T_{1u}^{}}_{L}^{A_{1g}^{}}_{L}^{E_{u}^{}}}$,
$d\indices*{*_{\Gamma}^{T_{1u}^{}}_{L}^{A_{2u}^{}}_{L}^{E_{g}^{}}}$,                                                                  
$\tensor*[^{0}]{d}{}\indices*{*_{\Gamma}^{T_{1u}^{}}_{L}^{E_{g}^{}}_{L}^{E_{u}^{}}}$,   
$\tensor*[^{1}]{d}{}\indices*{*_{\Gamma}^{T_{1u}^{}}_{L}^{E_{g}^{}}_{L}^{E_{u}^{}}}$,                                                 
$d\indices*{*_{\Gamma}^{T_{1u}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}A}{}_{1g}^{}}_{L}^{A_{2u}^{}}}$,
$d\indices*{*_{\Gamma}^{T_{1u}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}A}{}_{1g}^{}}_{L}^{E_{u}^{}}}$,      \\                       
$d\indices*{*_{\Gamma}^{T_{1u}^{}}_{L}^{A_{2u}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}}$,                                 
$\tensor*[^{0}]{d}{}\indices*{*_{\Gamma}^{T_{1u}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{L}^{E_{u}^{}}}$,   
$\tensor*[^{1}]{d}{}\indices*{*_{\Gamma}^{T_{1u}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{L}^{E_{u}^{}}}$
}\\
\\[-0.8em]
$(L,L,X)$ & 91 & \makecell{ 
$d\indices*{*_{L_{2}}^{A_{1g}^{}}_{L}^{A_{1g}^{}}_{X}^{A_{1g}^{}}}$,
$d\indices*{*_{L_{2}}^{A_{1g}^{}}_{L}^{E_{g}^{}}_{X}^{A_{1g}^{}}}$,
$\tensor*[^{1}]{d}{}\indices*{*_{L_{2}}^{A_{1g}^{}}_{L}^{E_{g}^{}}_{X}^{E_{g}^{}}}$, 
$\tensor*[^{0}]{d}{}\indices*{*_{L_{2}}^{A_{1g}^{}}_{L}^{E_{g}^{}}_{X}^{E_{g}^{}}}$,                                                  
$d\indices*{*_{L_{2}}^{A_{1g}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}A}{}_{1g}^{}}_{X}^{A_{1g}^{}}}$,  
$d\indices*{*_{L_{2}}^{A_{1g}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}A}{}_{1g}^{}}_{X}^{E_{g}^{}}}$, 
$d\indices*{*_{L_{2}}^{A_{1g}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{X}^{A_{1g}^{}}}$,                                  
$\tensor*[^{1}]{d}{}\indices*{*_{L_{2}}^{A_{1g}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{X}^{E_{g}^{}}}$, \\ 
$\tensor*[^{0}]{d}{}\indices*{*_{L_{2}}^{A_{1g}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{X}^{E_{g}^{}}}$, 
$d\indices*{*_{L_{2}}^{A_{1g}^{}}_{L}^{A_{2u}^{}}_{X}^{A_{2u}^{}}}$, 
$d\indices*{*_{L_{2}}^{A_{1g}^{}}_{L}^{A_{2u}^{}}_{X}^{B_{1u}^{}}}$,
$d\indices*{*_{L_{2}}^{A_{1g}^{}}_{L}^{A_{2u}^{}}_{X}^{E_{u}^{}}}$,
$d\indices*{*_{L_{2}}^{A_{1g}^{}}_{L}^{A_{2u}^{}}_{X}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}}$,
$d\indices*{*_{L_{2}}^{A_{1g}^{}}_{L}^{E_{u}^{}}_{X}^{A_{2u}^{}}}$, 
$d\indices*{*_{L_{2}}^{A_{1g}^{}}_{L}^{E_{u}^{}}_{X}^{B_{1u}^{}}}$, 
$\tensor*[^{0}]{d}{}\indices*{*_{L_{2}}^{A_{1g}^{}}_{L}^{E_{u}^{}}_{X}^{E_{u}^{}}}$,\\
$\tensor*[^{1}]{d}{}\indices*{*_{L_{2}}^{A_{1g}^{}}_{L}^{E_{u}^{}}_{X}^{E_{u}^{}}}$, 
$\tensor*[^{0}]{d}{}\indices*{*_{L_{2}}^{A_{1g}^{}}_{L}^{E_{u}^{}}_{X}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}}$,
$\tensor*[^{1}]{d}{}\indices*{*_{L_{2}}^{A_{1g}^{}}_{L}^{E_{u}^{}}_{X}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}}$,
$\tensor*[^{1}]{d}{}\indices*{*_{L_{2}}^{E_{g}^{}}_{L}^{E_{g}^{}}_{X}^{A_{1g}^{}}}$, 
$\tensor*[^{0}]{d}{}\indices*{*_{L_{2}}^{E_{g}^{}}_{L}^{E_{g}^{}}_{X}^{A_{1g}^{}}}$,
$d\indices*{*_{L_{2}}^{E_{g}^{}}_{L}^{E_{g}^{}}_{X}^{E_{g}^{}}}$,
$d\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}A}{}_{1g}^{}}_{L}^{E_{g}^{}}_{X}^{A_{1g}^{}}}$, 
$\tensor*[^{1}]{d}{}\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}A}{}_{1g}^{}}_{L}^{E_{g}^{}}_{X}^{E_{g}^{}}}$,   \\ 
$\tensor*[^{0}]{d}{}\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}A}{}_{1g}^{}}_{L}^{E_{g}^{}}_{X}^{E_{g}^{}}}$, 
$\tensor*[^{1}]{d}{}\indices*{*_{L_{2}}^{E_{g}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{X}^{A_{1g}^{}}}$,
$\tensor*[^{0}]{d}{}\indices*{*_{L_{2}}^{E_{g}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{X}^{A_{1g}^{}}}$,
$\tensor*[^{1}]{d}{}\indices*{*_{L_{2}}^{E_{g}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{X}^{E_{g}^{}}}$, 
$\tensor*[^{2}]{d}{}\indices*{*_{L_{2}}^{E_{g}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{X}^{E_{g}^{}}}$, 
$\tensor*[^{0}]{d}{}\indices*{*_{L_{2}}^{E_{g}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{X}^{E_{g}^{}}}$,
$\tensor*[^{3}]{d}{}\indices*{*_{L_{2}}^{E_{g}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{X}^{E_{g}^{}}}$,
$d\indices*{*_{L_{2}}^{E_{g}^{}}_{L}^{A_{2u}^{}}_{X}^{A_{2u}^{}}}$, \\
$d\indices*{*_{L_{2}}^{E_{g}^{}}_{L}^{A_{2u}^{}}_{X}^{B_{1u}^{}}}$,
$\tensor*[^{1}]{d}{}\indices*{*_{L_{2}}^{E_{g}^{}}_{L}^{A_{2u}^{}}_{X}^{E_{u}^{}}}$,
$\tensor*[^{0}]{d}{}\indices*{*_{L_{2}}^{E_{g}^{}}_{L}^{A_{2u}^{}}_{X}^{E_{u}^{}}}$,  
$\tensor*[^{1}]{d}{}\indices*{*_{L_{2}}^{E_{g}^{}}_{L}^{A_{2u}^{}}_{X}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}}$,
$\tensor*[^{0}]{d}{}\indices*{*_{L_{2}}^{E_{g}^{}}_{L}^{A_{2u}^{}}_{X}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}}$, 
$\tensor*[^{1}]{d}{}\indices*{*_{L_{2}}^{E_{g}^{}}_{L}^{E_{u}^{}}_{X}^{A_{2u}^{}}}$, 
$\tensor*[^{0}]{d}{}\indices*{*_{L_{2}}^{E_{g}^{}}_{L}^{E_{u}^{}}_{X}^{A_{2u}^{}}}$,    
$\tensor*[^{0}]{d}{}\indices*{*_{L_{2}}^{E_{g}^{}}_{L}^{E_{u}^{}}_{X}^{B_{1u}^{}}}$,      \\      
$\tensor*[^{1}]{d}{}\indices*{*_{L_{2}}^{E_{g}^{}}_{L}^{E_{u}^{}}_{X}^{B_{1u}^{}}}$,
$\tensor*[^{2}]{d}{}\indices*{*_{L_{2}}^{E_{g}^{}}_{L}^{E_{u}^{}}_{X}^{E_{u}^{}}}$,   
$\tensor*[^{0}]{d}{}\indices*{*_{L_{2}}^{E_{g}^{}}_{L}^{E_{u}^{}}_{X}^{E_{u}^{}}}$,   
$\tensor*[^{1}]{d}{}\indices*{*_{L_{2}}^{E_{g}^{}}_{L}^{E_{u}^{}}_{X}^{E_{u}^{}}}$,    
$\tensor*[^{3}]{d}{}\indices*{*_{L_{2}}^{E_{g}^{}}_{L}^{E_{u}^{}}_{X}^{E_{u}^{}}}$, 
$\tensor*[^{2}]{d}{}\indices*{*_{L_{2}}^{E_{g}^{}}_{L}^{E_{u}^{}}_{X}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}}$,
$\tensor*[^{0}]{d}{}\indices*{*_{L_{2}}^{E_{g}^{}}_{L}^{E_{u}^{}}_{X}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}}$, 
$\tensor*[^{1}]{d}{}\indices*{*_{L_{2}}^{E_{g}^{}}_{L}^{E_{u}^{}}_{X}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}}$,  \\ 
$\tensor*[^{3}]{d}{}\indices*{*_{L_{2}}^{E_{g}^{}}_{L}^{E_{u}^{}}_{X}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}}$, 
$d\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}A}{}_{1g}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}A}{}_{1g}^{}}_{X}^{A_{1g}^{}}}$,  
$d\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}A}{}_{1g}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{X}^{A_{1g}^{}}}$,
$\tensor*[^{1}]{d}{}\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}A}{}_{1g}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{X}^{E_{g}^{}}}$, 
$\tensor*[^{0}]{d}{}\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}A}{}_{1g}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{X}^{E_{g}^{}}}$,  
$d\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}A}{}_{1g}^{}}_{L}^{A_{2u}^{}}_{X}^{A_{2u}^{}}}$, 
$d\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}A}{}_{1g}^{}}_{L}^{A_{2u}^{}}_{X}^{B_{1u}^{}}}$,    
$d\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}A}{}_{1g}^{}}_{L}^{A_{2u}^{}}_{X}^{E_{u}^{}}}$,\\
$d\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}A}{}_{1g}^{}}_{L}^{A_{2u}^{}}_{X}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}}$,  
$d\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}A}{}_{1g}^{}}_{L}^{E_{u}^{}}_{X}^{A_{2u}^{}}}$, 
$d\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}A}{}_{1g}^{}}_{L}^{E_{u}^{}}_{X}^{B_{1u}^{}}}$,
$\tensor*[^{0}]{d}{}\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}A}{}_{1g}^{}}_{L}^{E_{u}^{}}_{X}^{E_{u}^{}}}$,   
$\tensor*[^{1}]{d}{}\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}A}{}_{1g}^{}}_{L}^{E_{u}^{}}_{X}^{E_{u}^{}}}$,
$\tensor*[^{0}]{d}{}\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}A}{}_{1g}^{}}_{L}^{E_{u}^{}}_{X}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}}$, 
$\tensor*[^{1}]{d}{}\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}A}{}_{1g}^{}}_{L}^{E_{u}^{}}_{X}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}}$, 
$\tensor*[^{1}]{d}{}\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{X}^{A_{1g}^{}}}$,  \\
$\tensor*[^{0}]{d}{}\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{X}^{A_{1g}^{}}}$,  
$d\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{L}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{X}^{E_{g}^{}}}$,
$d\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{L}^{A_{2u}^{}}_{X}^{A_{2u}^{}}}$,   
$d\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{L}^{A_{2u}^{}}_{X}^{B_{1u}^{}}}$,    
$\tensor*[^{1}]{d}{}\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{L}^{A_{2u}^{}}_{X}^{E_{u}^{}}}$, 
$\tensor*[^{0}]{d}{}\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{L}^{A_{2u}^{}}_{X}^{E_{u}^{}}}$, 
$\tensor*[^{1}]{d}{}\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{L}^{A_{2u}^{}}_{X}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}}$,
$\tensor*[^{0}]{d}{}\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{L}^{A_{2u}^{}}_{X}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}}$,  \\
$\tensor*[^{1}]{d}{}\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{L}^{E_{u}^{}}_{X}^{A_{2u}^{}}}$,  
$\tensor*[^{0}]{d}{}\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{L}^{E_{u}^{}}_{X}^{A_{2u}^{}}}$,
$\tensor*[^{0}]{d}{}\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{L}^{E_{u}^{}}_{X}^{B_{1u}^{}}}$,
$\tensor*[^{1}]{d}{}\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{L}^{E_{u}^{}}_{X}^{B_{1u}^{}}}$,
$\tensor*[^{2}]{d}{}\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{L}^{E_{u}^{}}_{X}^{E_{u}^{}}}$,  
$\tensor*[^{0}]{d}{}\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{L}^{E_{u}^{}}_{X}^{E_{u}^{}}}$,   
$\tensor*[^{1}]{d}{}\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{L}^{E_{u}^{}}_{X}^{E_{u}^{}}}$,    
$\tensor*[^{3}]{d}{}\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{L}^{E_{u}^{}}_{X}^{E_{u}^{}}}$,\\
$\tensor*[^{2}]{d}{}\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{L}^{E_{u}^{}}_{X}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}}$,
$\tensor*[^{0}]{d}{}\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{L}^{E_{u}^{}}_{X}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}}$,  
$\tensor*[^{1}]{d}{}\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{L}^{E_{u}^{}}_{X}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}}$,  
$\tensor*[^{3}]{d}{}\indices*{*_{L_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{g}^{}}_{L}^{E_{u}^{}}_{X}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}}$,  
$d\indices*{*_{L_{2}}^{A_{2u}^{}}_{L}^{A_{2u}^{}}_{X}^{A_{1g}^{}}}$,   
$d\indices*{*_{L_{2}}^{A_{2u}^{}}_{L}^{E_{u}^{}}_{X}^{A_{1g}^{}}}$,
$\tensor*[^{1}]{d}{}\indices*{*_{L_{2}}^{E_{u}^{}}_{L}^{A_{2u}^{}}_{X}^{E_{g}^{}}}$,
$\tensor*[^{0}]{d}{}\indices*{*_{L_{2}}^{E_{u}^{}}_{L}^{A_{2u}^{}}_{X}^{E_{g}^{}}}$,  \\
$\tensor*[^{1}]{d}{}\indices*{*_{L_{2}}^{E_{u}^{}}_{L}^{E_{u}^{}}_{X}^{A_{1g}^{}}}$,        
$\tensor*[^{0}]{d}{}\indices*{*_{L_{2}}^{E_{u}^{}}_{L}^{E_{u}^{}}_{X}^{A_{1g}^{}}}$,   
$d\indices*{*_{L_{2}}^{E_{u}^{}}_{L}^{E_{u}^{}}_{X}^{E_{g}^{}}}$
}\\
\\[-0.8em]
\fi
$(\Gamma,X,X)$ & 17 & \makecell{ 
$d\indices*{*_{\Gamma}^{T_{2g}^{}}_{X}^{A_{1g}^{}}_{X}^{E_{g}^{}}}$, 
$d\indices*{*_{\Gamma}^{T_{2g}^{}}_{X}^{A_{2u}^{}}_{X}^{E_{u}^{}}}$,
$d\indices*{*_{\Gamma}^{T_{2g}^{}}_{X}^{A_{2u}^{}}_{X}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}}$,  
$d\indices*{*_{\Gamma}^{T_{2g}^{}}_{X}^{B_{1u}^{}}_{X}^{E_{u}^{}}}$,
$d\indices*{*_{\Gamma}^{T_{2g}^{}}_{X}^{B_{1u}^{}}_{X}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}}$,
$d\indices*{*_{\Gamma}^{T_{2g}^{}}_{X}^{E_{g}^{}}_{X}^{E_{g}^{}}}$, 
$d\indices*{*_{\Gamma}^{T_{2g}^{}}_{X}^{B_{1u}^{}}_{X}^{A_{2u}^{}}}$,
$d\indices*{*_{\Gamma}^{T_{2g}^{}}_{X}^{E_{u}^{}}_{X}^{E_{u}^{}}}$,\\ 
$d\indices*{*_{\Gamma}^{T_{2g}^{}}_{X}^{E_{u}^{}}_{X}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}}$,  
$d\indices*{*_{\Gamma}^{T_{2g}^{}}_{X}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}_{X}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}}$,
$d\indices*{*_{\Gamma}^{T_{1u}^{}}_{X}^{A_{1g}^{}}_{X}^{E_{u}^{}}}$, 
$d\indices*{*_{\Gamma}^{T_{1u}^{}}_{X}^{A_{1g}^{}}_{X}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}}$,   
$d\indices*{*_{\Gamma}^{T_{1u}^{}}_{X}^{B_{1u}^{}}_{X}^{E_{g}^{}}}$,
$d\indices*{*_{\Gamma}^{T_{1u}^{}}_{X}^{E_{g}^{}}_{X}^{A_{2u}^{}}}$, 
$d\indices*{*_{\Gamma}^{T_{1u}^{}}_{X}^{A_{1g}^{}}_{X}^{A_{2u}^{}}}$,
$d\indices*{*_{\Gamma}^{T_{1u}^{}}_{X}^{E_{g}^{}}_{X}^{E_{u}^{}}}$, \\  
$d\indices*{*_{\Gamma}^{T_{1u}^{}}_{X}^{E_{g}^{}}_{X}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}}$,  
}\\
\\[-0.8em]
$(X,X,X)$ & 18 & \makecell{ 
$d\indices*{*_{X_{1}}^{A_{1g}^{}}_{X_{2}}^{A_{1g}^{}}_{X}^{A_{1g}^{}}}$, 
$d\indices*{*_{X_{1}}^{A_{1g}^{}}_{X_{2}}^{E_{g}^{}}_{X}^{E_{g}^{}}}$, 
$d\indices*{*_{X_{1}}^{A_{1g}^{}}_{X_{2}}^{A_{2u}^{}}_{X}^{E_{u}^{}}}$,
$d\indices*{*_{X_{1}}^{A_{1g}^{}}_{X_{2}}^{A_{2u}^{}}_{X}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}}$,
$d\indices*{*_{X_{1}}^{A_{1g}^{}}_{X_{2}}^{B_{1u}^{}}_{X}^{B_{1u}^{}}}$, 
$d\indices*{*_{X_{1}}^{A_{1g}^{}}_{X_{2}}^{E_{u}^{}}_{X}^{E_{u}^{}}}$,   
$d\indices*{*_{X_{1}}^{A_{1g}^{}}_{X_{2}}^{E_{u}^{}}_{X}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}}$,    
$d\indices*{*_{X_{1}}^{A_{1g}^{}}_{X_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}_{X}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}}$,\\
$d\indices*{*_{X_{1}}^{E_{g}^{}}_{X_{2}}^{E_{g}^{}}_{X}^{E_{g}^{}}}$,  
$d\indices*{*_{X_{1}}^{B_{1u}^{}}_{X_{2}}^{A_{2u}^{}}_{X}^{E_{g}^{}}}$,
$d\indices*{*_{X_{1}}^{B_{1u}^{}}_{X_{2}}^{E_{g}^{}}_{X}^{E_{u}^{}}}$, 
$d\indices*{*_{X_{1}}^{B_{1u}^{}}_{X_{2}}^{E_{g}^{}}_{X}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}}$,     
$d\indices*{*_{X_{1}}^{E_{g}^{}}_{X_{2}}^{E_{u}^{}}_{X}^{A_{2u}^{}}}$,
$d\indices*{*_{X_{1}}^{E_{g}^{}}_{X_{2}}^{E_{u}^{}}_{X}^{E_{u}^{}}}$, 
$\tensor*[^{0}]{d}{}\indices*{*_{X_{1}}^{E_{g}^{}}_{X_{2}}^{E_{u}^{}}_{X}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}}$,   
$d\indices*{*_{X_{1}}^{E_{g}^{}}_{X_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}_{X}^{A_{2u}^{}}}$,       \\
$\tensor*[^{1}]{d}{}\indices*{*_{X_{1}}^{E_{g}^{}}_{X_{2}}^{E_{u}^{}}_{X}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}}$,
$d\indices*{*_{X_{1}}^{E_{g}^{}}_{X_{2}}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}_{X}^{\tensor*[^{1}]{\hspace{-0.2em}E}{}_{u}^{}}}$
}\\
\\[-0.8em]
\end{tabular}
\end{ruledtabular}
